A More General Theory of Diagnosis from First Principles

Model-based diagnosis has been an active research topic in different communities including artificial intelligence, formal methods, and control. This has led to a set of disparate approaches addressing different classes of systems and seeking different forms of diagnoses. In this paper, we resolve such disparities by generalising Reiter's theory to be agnostic to the types of systems and diagnoses considered. This more general theory of diagnosis from first principles defines the minimal diagnosis as the set of preferred diagnosis candidates in a search space of hypotheses. Computing the minimal diagnosis is achieved by exploring the space of diagnosis hypotheses, testing sets of hypotheses for consistency with the system's model and the observation, and generating conflicts that rule out successors and other portions of the search space. Under relatively mild assumptions, our algorithms correctly compute the set of preferred diagnosis candidates. The main difficulty here is that the search space is no longer a powerset as in Reiter's theory, and that, as consequence, many of the implicit properties (such as finiteness of the search space) no longer hold. The notion of conflict also needs to be generalised and we present such a more general notion. We present two implementations of these algorithms, using test solvers based on satisfiability and heuristic search, respectively, which we evaluate on instances from two real world discrete event problems. Despite the greater generality of our theory, these implementations surpass the special purpose algorithms designed for discrete event systems, and enable solving instances that were out of reach of existing diagnosis approaches.

==> imple.tex <==
In this section, we show how the algorithms 
presented in this article can be concretely implemented.  
We illustrate the test solvers 
and the modeling of the hypothesis properties 
for the diagnosis of circuits and the diagnosis of DES.  
This requires to explain 
1) how to represent the model and the observation, 
2) how to represent a set of properties and each property, 
and 3) how to generate conflicts.  

\subsection{Diagnosis of Boolean Circuits}

A possible implementation of a tester for Boolean circuits 
is the reduction to SAT \cite{metodi-etal::aaai::12}.  
A SAT problem is derived from the test $\langle \MOD, o, H\rangle$, 
that is satisfiable iff the test is successful.  

The SAT formula is the conjunction of three formulas 
which respectively represent the model, the observation, 
and the set of hypotheses $H$.  
The translation of the model is trivial; 
for instance, if the and gate $A$ has inputs $i_1$ and $i_2$ 
and output $o$, then the following formula is included in the SAT problem: 
$\neg \verb+ab_+A \rightarrow (\verb+o+ = \verb+i1+ \land \verb+i2+)$ 
where $\verb+ab_+A$ is the health variable of component $A$.  
The translation of the observation is also trivial; 
for instance, if the output $o$ is observed to be $\bot$, 
the following unit clause is added to the SAT problem: 
$\neg \verb+o+$.  

The hypothesis space considered for Boolean circuits 
is generally SHS.  
A hypothesis of this space is a set of abnormal components 
while the other components' state is assumed nominal.  
Hence, let $C$ be the set of components 
and $h \subseteq C$ be a hypothesis; 
the hypothesis $h$ is translated to SAT 
as the following conjunction: 
\begin{displaymath}
  \bigwedge_{c \in h} (\verb+ab_+c) 
  \land 
  \bigwedge_{c \in C \setminus h} (\neg \verb+ab_+c)
\end{displaymath}

The SAT formula associated with a set of hypothesis properties 
is the conjunction of the formulas associated with each property.  

Property $\propdesc(h)$ represents the set of descendants of $h$, 
i.e., all hypotheses that assume that all components of $h$ are faulty.  
This can be expressed by 
$\bigwedge_{c \in h} (\verb+ab_+c)$.  
The opposite property, $\neg\propdesc(h)$, 
can be expressed by $\bigvee_{c \in h} (\neg \verb+ab_+c)$.  

Property $\propanc(h)$ represents the set of ancestors of $h$, 
i.e., all hypotheses that assume 
that no components outside $h$ is faulty.   
This can be expressed by 
$\bigwedge_{c \in C \setminus h} (\neg \verb+ab_+c)$.  
The opposite property, $\\neg\propanc(h)$, 
can be expressed by $\bigvee_{c \in C \setminus h} (\verb+ab_+c)$.  

The most efficient complete SAT solvers 
implement conflict directed clause learning (CDCL) 
\cite{moskewicz-etal::dac::01}.  
Such algorithms can take as input a set of assumptions and, 
if the conjunction of these assumptions and the SAT problem 
are unsatisfiable, 
return a subset of assumptions sufficient for unsatisfiability.  
The SAT representation of the properties described above 
can be given as assumptions; 
the CDCL procedure will then return a diagnostic conflict 
if the test fails.  

\subsection{Diagnosis of Discrete Event Systems}

A test for the diagnosis of discrete event systems 
can be seen as a model-checking problem 
formulated as follows: \textit{Does the model allow 
for a sequence of transitions that generates the actual observation 
and satisfies the hypothesis properties?}  
Such a tester can be implemented 
using model-checking or classical planning techniques 
\cite{sohrabi-etal::kr::10,haslum-grastien::spark::11}.  
We now present this problem 
as the problem of determining language emptiness.  

Given the set $\Sigma$ of events, 
we define three languages: 
$\mathcal{L}_M$ is the set of sequences of events (aka words) 
that may occur on the system according to the model; 
$\mathcal{L}_O$ is the set of words 
that are consistent with the observation 
(if the observation is a word, 
then $\mathcal{L}_O$ is the set of words 
whose projection on the set $\Sigma_O$ of observable events 
is the actual observation); 
and $\mathcal{L}_H$ is the set of words 
whose corresponding hypothesis belongs to $H$.  
Both $\mathcal{L}_O$ and $\mathcal{L}_H$ 
generally contain words that are forbidden by $\mathcal{L}_M$.  
Following the reduction to model-checking given above, 
a test is successful 
if and only if the intersection of the three languages is not empty.  

Let us now concentrate on the representation of $\mathcal{L}_H$.  
Assume we are now dealing with SeqHS hypothesis space.  
Let $F$ be the set of faults 
and let $h = [f_1,\dots,f_k] \in F^\star$ be a hypothesis 
(where the same fault $f$ may appear several times, 
e.g., $f = f_i = f_j$, $i \neq j$) 
The language $\mathcal{L}_h$ 
representing the words that correspond to hypothesis $h$ 
is 
\begin{displaymath}
  (\Sigma \setminus F)^\star\ f_1\ (\Sigma \setminus F)^\star\ f_2 \
  \dots \
  f_{k-1}\ (\Sigma \setminus F)^\star\ f_k\ (\Sigma \setminus F)^\star .  
\end{displaymath}

The language associated with a set of hypothesis properties 
is the intersection of the languages associated with each property.  

Property $\propdesc(h)$ represents the set of descendants of $h$, 
i.e., all hypotheses that assume that all faults in $h$ occurred 
in this order (with possibly more faults).  
This can be expressed by 
\begin{displaymath}
  \Sigma^\star\ f_1\ \Sigma^\star\ f_2 \
  \dots \
  f_{k-1}\ \Sigma^\star\ f_k\ \Sigma^\star.  
\end{displaymath}
The opposite property, $\neg\propdesc(h)$, 
can be expressed by $\Sigma^\star \setminus \mathcal{L}_{\propdesc(h)}$.  

Property $\propanc(h)$ represents the set of ancestors of $h$, 
i.e., all hypotheses that assume 
that the only faulty events that may have occurred 
are those that appear in $h$, in this order.  
This can be expressed by 
\begin{displaymath} 
  (\Sigma \setminus F)^\star\ f_1^{0/1}\ (\Sigma \setminus F)^\star\ f_2^{0/1} \
  \dots \
  f_{k-1}?\ (\Sigma \setminus F)^\star\ f_k^{0/1}\ (\Sigma \setminus F)^\star.  
\end{displaymath}
The opposite property, $\neg\propanc(h)$, 
can be expressed by $\Sigma^\star \setminus \mathcal{L}_{\propanc(h)}$.  

The conflict extraction is more difficult in this setting.  
The goal is to find a subset of the hypothesis property languages 
whose intersection with $\mathcal{L}_M$ and $\mathcal{L}_O$ is empty.  

If the intersection $\mathcal{L}_M \cap \mathcal{L}_O 
\cap \mathcal{L}_{p_1} \cap \dots \cap \mathcal{L}_{p_k}$ 
is performed incrementally, 
then, as soon as an empty set is generated 
(say, after the synchronisation with $\mathcal{L}_i$), 
a conflict is discovered (in this example, $\{p_1,\dots,p_i\}$).  

There is some work in classical planning 
to find conflict, but I think Patrik should write this bit.  

Finally, a successful approach for classical planning 
is the reduction to SAT.  
CDCL techniques described for Boolean circuits 
can also be used in such a situation.  

% EOF


==> tab.tex <==
\begin{longtable}{| c || c || c || c | c | c | c |}
Problem & JT & BDD & SAT set & SAT set-tight & SAT multiset & SAT seq \\
chunk-004 & 3.1 & {\bf 0.2} & 0.6 & 0.6 & 0.7 & 0.6 \\
chunk-008 & 3.8 & {\bf 0.3} & 0.6 & 0.6 & 0.6 & 0.6 \\
chunk-026 & --T-- & {\bf 4.7} & 6.2 & 5.6 & 6.1 & 8.7 \\
chunk-037 & --T-- & {\bf 1.8} & 3.5 & 3.3 & 5.1 & 6.9 \\
chunk-040 & --T-- & {\bf 0.7} & 1.1 & 1.1 & 1.2 & 1.6 \\
chunk-045 & --T-- & 22.9 & 13.3 & 13.5 & {\bf 12.8} & 14.4 \\
chunk-049 & --T-- & {\bf 6.3} & 7.0 & 6.7 & 6.9 & 16.8 \\
chunk-054 & --T-- & {\bf 2.0} & 2.5 & 2.7 & 2.4 & 2.3 \\
chunk-056 & 3.4 & {\bf 0.3} & 1.1 & 1.0 & 1.2 & 1.4 \\
chunk-073 & 3.4 & {\bf 0.3} & 0.9 & 0.9 & 0.9 & 0.9 \\
chunk-076 & --T-- & 6.8 & {\bf 6.3} & 7.7 & 9.2 & 131.7 \\
chunk-077 & --T-- & {\bf 4.9} & 5.6 & 5.4 & 5.1 & 6.2 \\
chunk-078 & --T-- & {\bf 8.5} & 11.0 & 15.7 & 19.8 & 362.8 \\
chunk-089 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
chunk-091 & --T-- & {\bf 41.2} & 250.2 & 231.5 & 409.6 & --T-- \\
chunk-105 & --T-- & 1.4 & {\bf 1.1} & {\bf 1.1} & 1.5 & 3.1 \\
chunk-111 & --T-- & {\bf 44.8} & 97.5 & 116.5 & 195.6 & --T-- \\
chunk-127 & --T-- & {\bf 1.0} & 1.7 & 1.7 & 1.9 & 3.0 \\
chunk-132 & --T-- & 20.2 & {\bf 4.2} & {\bf 4.2} & 5.3 & 6.8 \\
chunk-133 & --T-- & 3.0 & {\bf 2.6} & 3.0 & 3.3 & 4.1 \\
window-006 & 2.9 & {\bf 0.3} & 0.7 & 0.6 & 0.6 & 2.4 \\
window-007 & 2.9 & {\bf 0.3} & 0.5 & 0.4 & 0.4 & 0.5 \\
window-013 & 3.5 & {\bf 0.3} & 0.6 & 0.6 & 0.6 & 0.6 \\
window-015 & 2.9 & {\bf 0.3} & 0.5 & 0.5 & 0.5 & 0.5 \\
window-053 & --T-- & 1.6 & 1.2 & {\bf 1.1} & {\bf 1.1} & 1.2 \\
window-055 & --T-- & 1.8 & {\bf 1.1} & {\bf 1.1} & {\bf 1.1} & {\bf 1.1} \\
window-057 & --T-- & 1.6 & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} \\
window-093 & 3.3 & {\bf 0.4} & 0.9 & 0.9 & 0.9 & 1.0 \\
window-095 & 3.2 & {\bf 0.4} & 0.9 & 0.8 & 0.8 & 0.9 \\
window-096 & 2.8 & {\bf 0.2} & 0.6 & 0.5 & 0.5 & 0.5 \\
window-098 & 3.0 & {\bf 0.3} & 0.7 & 0.7 & 0.7 & 0.7 \\
window-115 & --T-- & {\bf 0.7} & 1.1 & 1.1 & 1.2 & 1.7 \\
window-116 & --T-- & {\bf 0.7} & {\bf 0.7} & {\bf 0.7} & {\bf 0.7} & {\bf 0.7} \\
window-124 & --T-- & 17.7 & {\bf 8.7} & 8.8 & 9.1 & 9.8 \\
window-125 & --T-- & 17.2 & 10.4 & {\bf 10.0} & 10.5 & 12.6 \\
window-126 & --T-- & 13.8 & 7.5 & 7.6 & {\bf 7.2} & 8.2 \\
window-127 & --T-- & 15.0 & 8.4 & {\bf 8.1} & 8.3 & 10.0 \\
window-128 & --T-- & 13.1 & 5.8 & 6.0 & {\bf 5.6} & 6.6 \\
window-129 & --T-- & 10.4 & {\bf 3.6} & 3.8 & {\bf 3.6} & 4.3 \\
window-130 & --T-- & 10.0 & 5.8 & {\bf 5.5} & 5.6 & 7.3 \\
window-131 & --T-- & 11.2 & {\bf 3.4} & 3.7 & {\bf 3.4} & 3.8 \\
window-132 & --T-- & 10.8 & 5.2 & {\bf 5.0} & 5.1 & 7.8 \\
window-133 & --T-- & 9.4 & 3.0 & {\bf 2.9} & 3.1 & 3.4 \\
window-134 & --T-- & 9.9 & 3.5 & 3.7 & {\bf 3.4} & 4.8 \\
window-135 & --T-- & 1.5 & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} \\
window-136 & --T-- & 1.5 & 1.2 & {\bf 1.1} & {\bf 1.1} & 1.3 \\
window-137 & 2.4 & {\bf 0.2} & 0.4 & 0.3 & 0.3 & 0.4 \\
window-155 & --T-- & 3.1 & 2.0 & {\bf 1.9} & {\bf 1.9} & 2.8 \\
window-157 & --T-- & 2.5 & {\bf 1.3} & {\bf 1.3} & {\bf 1.3} & 1.8 \\
window-158 & 3.2 & {\bf 0.3} & 0.5 & 0.5 & 0.5 & 0.5 \\
window-173 & --T-- & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} \\
window-174 & --T-- & {\bf 1.0} & 1.2 & 1.1 & 1.2 & 1.3 \\
window-175 & --T-- & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} & {\bf 1.0} \\
window-177 & 2.3 & {\bf 0.2} & 0.3 & 0.3 & 0.3 & 0.4 \\
window-183 & --T-- & {\bf 1.1} & 1.2 & {\bf 1.1} & {\bf 1.1} & 1.2 \\
window-184 & --T-- & {\bf 1.1} & 1.5 & 1.4 & 1.4 & 1.6 \\
window-185 & --T-- & {\bf 0.9} & {\bf 0.9} & {\bf 0.9} & {\bf 0.9} & 1.0 \\
window-186 & --T-- & {\bf 0.8} & 1.1 & 1.0 & 1.1 & 1.2 \\
window-187 & --T-- & 0.9 & {\bf 0.8} & {\bf 0.8} & {\bf 0.8} & {\bf 0.8} \\
window-188 & --T-- & {\bf 0.9} & 1.0 & 1.0 & 1.0 & 1.2 \\
window-193 & 2.8 & {\bf 0.3} & 0.6 & 0.6 & 0.6 & 0.7 \\
window-194 & 2.9 & {\bf 0.2} & 0.5 & 0.5 & 0.5 & 0.6 \\
window-247 & 2.9 & {\bf 0.3} & 0.9 & 0.9 & 0.9 & 1.0 \\
window-248 & 2.9 & {\bf 0.3} & 0.9 & 0.9 & 0.9 & 1.4 \\
window-249 & 3.0 & {\bf 0.3} & 0.8 & 0.7 & 0.7 & 0.8 \\
window-250 & 2.3 & {\bf 0.2} & 0.3 & 0.3 & 0.3 & 0.3 \\
window-256 & --T-- & 7.5 & {\bf 6.5} & 7.6 & 9.1 & 133.3 \\
window-257 & --T-- & 7.1 & {\bf 4.0} & 6.0 & 6.2 & 87.4 \\
window-258 & --T-- & 6.4 & {\bf 3.3} & 4.9 & 5.0 & 101.6 \\
window-261 & --T-- & {\bf 1.9} & 2.3 & 2.7 & 2.3 & 2.7 \\
window-273 & --T-- & {\bf 7.9} & 8.9 & 12.4 & 14.6 & 226.7 \\
window-274 & --T-- & 7.1 & {\bf 6.6} & 10.3 & 12.0 & 213.8 \\
window-275 & --T-- & {\bf 4.2} & 6.6 & 6.3 & 7.2 & 23.9 \\
window-276 & --T-- & {\bf 4.2} & 5.0 & 4.9 & 5.7 & 15.0 \\
window-277 & --T-- & {\bf 4.1} & 4.3 & 4.2 & 4.3 & 12.8 \\
window-278 & --T-- & 4.2 & {\bf 3.2} & {\bf 3.2} & {\bf 3.2} & 8.3 \\
window-317 & --T-- & {\bf 3.4} & 5.2 & 7.7 & 17.3 & 221.5 \\
window-318 & --T-- & {\bf 5.3} & 15.0 & 14.0 & 27.4 & --T-- \\
window-319 & --T-- & {\bf 5.3} & 14.5 & 13.0 & 23.5 & --T-- \\
window-320 & --T-- & {\bf 5.3} & 12.5 & 12.1 & 20.0 & --T-- \\
window-321 & --T-- & {\bf 4.8} & 11.6 & 11.1 & 16.5 & --T-- \\
window-322 & --T-- & {\bf 5.4} & 10.4 & 10.4 & 13.6 & 596.0 \\
window-323 & --T-- & {\bf 5.3} & 9.8 & 9.3 & 10.8 & 424.8 \\
window-324 & --T-- & {\bf 4.7} & 9.1 & 8.8 & 8.6 & 405.5 \\
window-325 & --T-- & {\bf 5.8} & 10.7 & 15.3 & 18.8 & --T-- \\
window-330 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-331 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-332 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-333 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-334 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-335 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-336 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-337 & --T-- & --T-- & --T-- & --T-- & --T-- & --T-- \\
window-338 & --T-- & --T-- & --T-- & {\bf 380.0} & --T-- & --T-- \\
window-339 & --T-- & --T-- & --T-- & {\bf 335.1} & --T-- & --T-- \\
window-340 & --T-- & --T-- & --T-- & {\bf 332.0} & --T-- & --T-- \\
window-341 & --T-- & --T-- & --T-- & {\bf 310.4} & --T-- & --T-- \\
window-342 & --T-- & --T-- & --T-- & {\bf 271.6} & 538.6 & --T-- \\
window-343 & --T-- & --T-- & --T-- & {\bf 229.9} & 412.7 & --T-- \\
window-344 & --T-- & --T-- & 110.3 & {\bf 108.6} & 156.5 & --T-- \\
window-345 & --T-- & --T-- & {\bf 71.6} & 73.4 & 113.7 & --T-- \\
window-346 & --T-- & --T-- & 64.7 & {\bf 63.8} & 93.8 & --T-- \\
window-347 & --T-- & --T-- & 38.3 & {\bf 37.8} & 63.5 & 209.6 \\
window-348 & --T-- & 40.9 & {\bf 18.6} & {\bf 18.6} & 26.0 & 50.7 \\
window-349 & --T-- & 14.6 & 8.4 & {\bf 8.2} & 11.3 & 17.8 \\
window-350 & --T-- & 14.7 & {\bf 10.2} & 10.3 & 11.6 & 16.6 \\
window-351 & --T-- & 13.5 & {\bf 9.6} & 9.7 & 11.1 & 15.9 \\
window-352 & --T-- & 8.6 & 7.3 & {\bf 7.0} & 8.4 & 11.4 \\
window-353 & --T-- & {\bf 5.5} & {\bf 5.5} & 5.7 & 6.4 & 8.4 \\
window-366 & --T-- & {\bf 7.6} & 16.1 & 15.3 & 15.6 & 364.7 \\
window-367 & --T-- & {\bf 11.3} & 28.8 & 22.1 & 23.9 & 303.1 \\
window-368 & --T-- & {\bf 17.3} & 22.4 & 21.9 & 22.7 & 291.6 \\
window-369 & --T-- & {\bf 17.6} & 18.4 & 18.9 & 18.9 & 106.6 \\
window-370 & --T-- & 18.1 & {\bf 16.3} & 17.5 & 17.6 & 62.4 \\
window-371 & --T-- & 18.0 & {\bf 17.4} & 17.9 & 18.2 & 94.8 \\
window-409 & {\bf 7.2} & 22.3 & 138.1 & 153.8 & 257.9 & --T-- \\
window-410 & {\bf 6.9} & 11.7 & 53.8 & 64.3 & 94.2 & --T-- \\
window-506 & --T-- & 1.4 & 1.1 & {\bf 1.0} & 1.6 & 3.2 \\
window-524 & --T-- & {\bf 3.3} & 4.5 & 4.4 & 7.2 & 12.2 \\
window-525 & --T-- & {\bf 3.2} & 4.1 & 4.6 & 5.3 & 8.8 \\
window-526 & --T-- & {\bf 3.3} & 3.8 & 3.7 & 3.8 & 5.7 \\
window-527 & --T-- & 2.9 & 2.8 & {\bf 2.7} & 2.8 & 3.1 \\
window-601 & --T-- & {\bf 0.6} & 0.9 & 0.9 & 0.9 & 1.0 \\
window-602 & --T-- & {\bf 0.7} & {\bf 0.7} & {\bf 0.7} & {\bf 0.7} & 0.8 \\
window-617 & --T-- & 4.9 & {\bf 1.4} & {\bf 1.4} & {\bf 1.4} & 1.6 \\
window-618 & --T-- & 0.8 & 0.7 & {\bf 0.6} & 0.7 & 0.7 \\
window-620 & --T-- & 2.5 & {\bf 1.2} & {\bf 1.2} & {\bf 1.2} & 1.3 \\
window-622 & --T-- & 2.9 & {\bf 1.6} & {\bf 1.6} & 2.1 & 2.4 \\
window-623 & --T-- & 2.7 & 1.9 & {\bf 1.8} & 1.9 & 1.9 \\
\hline
129 & 23 & 110 & 114 & 120 & 116 & 102 \\
\end{longtable}

